XD at SemEval-2020 Task 12: Ensemble Approach to Offensive Language Identification in Social Media Using Transformer Encoders

This paper presents six document classification models using the latest transformer encoders and a high-performing ensemble model for a task of offensive language identification in social media. For the individual models, deep transformer layers are applied to perform multi-head attentions. For the ensemble model, the utterance representations taken from those individual models are concatenated and fed into a linear decoder to make the final decisions. Our ensemble model outperforms the individual models and shows up to 8.6% improvement over the individual models on the development set. On the test set, it achieves macro-F1 of 90.9% and becomes one of the high performing systems among 85 participants in the sub-task A of this shared task. Our analysis shows that although the ensemble model significantly improves the accuracy on the development set, the improvement is not as evident on the test set.

==> tex/approach.tex <==
\section{Approach}
\label{sec:approach}

Default transformer-based models are fine-tuned as baseline models on the dataset. Then we pre-train these default models on the total dataset and choose the models with lowest perplexity. Next we fine-tune them into regression models and classification models based on corresponding dataset. Furthermore, the regression models and classification models are finetuned again into classification models. In the end, we ensemble the models which have high performance on the development set.






% First, we will fine-tune the existed state-of-art language model, like Albert, for classification on the dataset as our baseline model. Because each dataset may be noisy to some extent, to use the dataset more efficiently and caputure the information in the dataset better, we assume the labels of the data which have high confidence are trustful and can be used to train the classification model. Thus, the classification model can learn a clear representation from these data. Then, for data with least confidence, we implement a simulation of the query process in which the model will query the labels of data with least confidence for training in active learning methodology. It means that we will use a regression model to capture the uncertainty in these least confidence data. Finally, we will joint the classification model which is trained on the data with high confidence and the regression model which is trained on the data with least confidence together for further prediction. 

% Joint learning has been widely applied in computer vision area, like image classification, learning auto-encoders, image generation~\cite{zhang-etal:2019},pedestrian detection~\cite{ouyang-wang:2013}, and in natural language processing area, like machine translation~\cite{bahdanau-etal:2014,garg-etal:2019}, sentiment classification~\cite{yu-jiang:2016} and emotion classification~\cite{chen-etal:2018}, extractive query-focused summarization~\cite{cao-etal:2016}, named entity recognition~\cite{nosirova:2019} and entity linking~\cite{martins-etal:2019},entity and event coreference resolution~\cite{barhom-etal:2019}, parser~\cite{duong-etal:2015,ye-etal:2019}, semantic representation~\cite{liu-etal:2015}, sequence labeling~\cite{rei:2017},dialog act segmentation and recognition~\cite{zhao-kawahara:2017,zhao-kawahara:2018}.

% There are two joint learning methods for deep learning, the hard parameter sharing and the soft parameter sharing~\cite{ruder:2017a}. We use the hard parameter sharing for our joint learning model, which means that it shares the hidden layers for both the classification model and the regression model while keeps the different task-specific output layers. Because dataset for each task are full of noise to some extent, when training a model on every individual task, it only learns a good representation on this task and ignores the data-dependent noise. And it may have the risk of being overfitting on this task. However, by applying the joint learning between models trained on different tasks, the model can find a more proper presentation which can capture information of both of the tasks and average the noise patterns, so it can get a global representation and reduce the risk of model overfitting on the original task.


